Attack-resistant Spanning Tree Construction in Route-Restricted Overlay Networks

Nodes in route-restricted overlays have an immutable set of neighbors, explicitly specified by their users. Popular examples include payment networks such as the Lightning network as well as social overlays such as the Dark Freenet. Routing algorithms are central to such overlays as they enable communication between nodes that are not directly connected. Recent results show that algorithms based on spanning trees are the most promising provably efficient choice. However, all suggested solutions fail to address how distributed spanning tree algorithms can deal with active denial of service attacks by malicious nodes. In this work, we design a novel self-stabilizing spanning tree construction algorithm that utilizes cryptographic signatures and prove that it reduces the set of nodes affected by active attacks. Our simulations substantiate this theoretical result with concrete values based on real-world data sets. In particular, our results indicate that our algorithm reduces the number of affected nodes by up to 74% compared to state-of-the-art attack-resistant spanning tree constructions.

==> background.tex <==
\srch{}{In this paper, we apply concepts from the area of self-stabilization to route-restricted overlays. Hence, we now introduce key notions from both areas. }
\subsection{Route-restricted overlays}
\srch{More generally, we refer to}{We define} an \emph{overlay network}, or just overlay, as a network between multiple logically connected nodes that communicate via a public infrastructure such as the Internet.
In \emph{route-restricted overlays}, the logical connections between nodes are explicitly managed by their respective users\srch{, such that the setup of a new connection between two nodes requires prior permission by their user.}{and hard or even impossible to adapt to a topology that benefits routing.}

More specifically, our work addresses the following two special cases of route-restricted overlays:
\sr{A bit repetitive to intro, not enough about why we need attack resilience}
\paragraph{Payment channel Networks}
Payment channel networks~\cite{poon2016lightning,malavolta2017silentwhispers,raiden2019} form an addendum to Blockchain-based digital payment systems to overcome their insufficient transaction rate.
Instead of adding every transaction to the Blockchain, a user $A$ that wants to send payments to a merchant $B$ instead only adds two transactions: one to open the channel and another to close it, thereby settling the final balance.
Between these two transactions, $A$ can send an arbitrary number of payments to $B$ directly, without interacting with the Blockchain.
The logical connections in the resulting route-restricted overlay thus represent the currently open payment channels between the participating nodes. 


\srch{To reduce the number of concurrently open channels, payment networks allow the settling of payments via existing channels.
If a user $A$ wants to pay a merchant $B$ and there exists a path with sufficient funds between $A$ and $B$ in the overlay, then $A$ can send funds along this path instead to settle the payment.}{Nodes $A$ and $B$ without an open channel between them can send the payment along one or multiple paths of channels.}
A routing algorithm that finds suitable overlay paths \srch{quickly}{to conduct payments} is thus essential for the practical usefulness of payment channel networks.

\paragraph{Social Overlays}
In a social overlay network or Friend-to-Friend network, like the Dark Freenet~\cite{clarke2010private}, the logical connections between overlay nodes correspond to the mutual trust relationships between their respective users.
To establish an overlay connection, both users typically exchange contact information out of band (e.g. via QR codes or text files).

In the context of censorship circumvention, social overlays play an important role for the implementation of membership concealing overlay networks~\cite{vasserman2009} that make it difficult for the censor to identify and monitor the overlay's participants.
Furthermore, social overlays are considered to be more robust against Sybil attacks~\cite{douceur2002sybil} because the setup of logical connections requires prior social engineering of the corresponding users.
For example, X-Vine~\cite{mittal2012}, GNUnet~\cite{grothoff2017gnunet} and Pisces~\cite{mittal2013pisces} employ social overlays to increase resilience against sybil attacks.
An efficient and privacy-preserving routing algorithm enables anonymous publishing as well as pseudonymous communication over social overlays.

\subsection{Topology-aware self-stabilization}
\label{sec:stabilization}
\sr{do we really need this here? we have a formal def later on, maybe we can add a sentence to the intro about relying on the concept of Topology-aware self-stabilization in the proofs and adding a shorter informal definition there}
Informally, a distributed system is said to be \emph{self-stabilizing} if, regardless of the initial state of each node, it reaches a \emph{legitimate state}, where every node has set its internal variables correctly, in a finite amount of time.
After the system has reached a legitimate state, it will remain so as long as no fault occurs.

To formalize the convergence of a distributed algorithm in the presence of Byzantine behavior, Dubois et al.~\cite{dubois2010byzantine} introduced \emph{topology-aware (TA) strict stabilization}.
Informally, a distributed system is $S_B$-TA strictly stabilizing if all non-Byzantine nodes except a subset $S_B$ will eventually reach a correct state and remain correct, irrespective of the actions of Byzantine nodes.
The subset $S_B$ is usually clearly defined in terms of structure, e.g., all nodes within a certain distance of a Byzantine node. 
The key idea is that nodes outside of $S_B$ might initially act based on incorrect information provided by Byzantine nodes but will eventually disregard such information.
For instance, $u \notin S_B$ might initially accept a Byzantine node's claims to be the root node in a distributed spanning tree.
However, once it receives a message from the correct root node, it will change accordingly.
Note that we do allow for the node to alternate between correct and incorrect states initially as long as it reaches a final correct state after a bounded number of changes.    
For example, Dubois et al.~\cite{dubois2010byzantine} present a protocol for the computation of a BFS spanning tree that, given a dedicated root node, is TA strictly stabilizing for $S_B = \{ v \in H \mid d_S(v,r) < \min_{b \in B} d_S(v,b)\}$ with $d_S(u,v)$ being the hop distance between $u$ and $v$ in an overlay $S$.


==> optimizations.tex <==
\section{Reducing overhead}

\paragraph{Aggregate signatures}
To reduce the number of signatures within a level attestation, an aggregate signature scheme can be used.
Instead of appending a new signature with every step, an attestation includes only one aggregate signature that is updated accordingly at each hop.

\paragraph{Hash chains}
If an upper bound $diam$ on the network diameter is known, hash chains can be used instead of our level attestations as follows:
\begin{enumerate}
   \item The root node picks a random number $r$ and uses a cryptographic hash function $H$ repeatedly to produce a sequence $h_1=H(r),h_2=H(h_1),\dots,h_{diam}$
   \item The value $h_{diam}$ replaces the globally known public key assumed by our attestation protocol
   \item For each neighbor $u$ with distance $d(r,u)$, $r$ hashes $h_1$ $d(r,u)$ times and sends the result to $u$
   \item To obtain the distance value associated with a hash value $h$, the node hashes $h$ until $h_{diam}$ has been produced. If this took $k$ hashing-operations, then the distance value is $diam-k$.
\end{enumerate}
When used for payment channel networks, $h_{diam}$ stands for a capacity of $0$ whereas $h_1$ stands for the maximum channel capacity.
However, this approach has the following drawbacks:
\begin{itemize}
   \item It does not offer loop detection.
   \item It does not provide replay protection (which we provide by the timestamps)
\end{itemize}
Hu et al.~\cite{hu2003sead} present a secure version of the Destination-Sequenced Distance-vector ad hoc network routing protocol that uses hash chains to protect distance values.\martin{However, I'm not sure if they provide loop detection caused by a link/node failure, because the node observing the link failure is not permitted to change the sequence number associated with the neighbor. Thus, their protocol might not be self-stabilizing.}

